LCDN: Providing Network Determinism with Low-Cost Switches

The demands on networks are increasing at a fast pace. In particular, real-time applications have very strict network requirements. However, building a network that hosts real-time applications is a cost-intensive endeavor, especially for experimental systems such as testbeds. Systems that provide guaranteed real-time networking capabilities usually work with expensive software-defined switches. In contrast, real-time networking systems based on low-cost hardware face the limitation of lower link speeds. This paper fills this gap and presents Low-Cost Deterministic Networking (LCDN), a system designed to work with inexpensive, common off-the-shelf switches and devices. LCDN works at Gigabit speed and enables powerful testbeds to host real-time applications with strict delay guarantees. This paper also provides an evaluation of the determinism of the switch and a Raspberry Pi used as an end device to demonstrate the applicability of LCDN on inexpensive low-power reduced capacity apparatus.

==> Writing/Results.tex <==
\section{Discussion on Limitations}
\label{sec:limits}

LCDN is designed to work with relatively low-cost hardware. In this initial setup, LCDN works with the FS S2805S switch series, which starts at around 85 €, and the Raspberry Pi 4, which is in a similar price range. Clearly, these devices come with limitations. These limitations, on the one side, decrease the performance of LCDN compared to larger data-center-focused systems like Chameleon \cite{van_bemten_chameleon_2020}. On the other side, the limitations also help LCDN, especially when looking at the routing. For example, LCDN uses a single VLAN-Tag to route the packet through the network. In total, there are 4094 usable VLAN-Tags, which limit the number of flows. However, when using lower-powered end hosts, LCDN does not expect to exhaust the number of VLAN-Tags and all possible routes. Another limitation is the number of MAC-Addresses a switch can use, which is 8000 MAC-Addresses per switch.

LCDN expects that the networks and setups it uses are of reasonable size and within the capabilities of the switches and end hosts. 
 

